Causality-Aided Falsification

Falsification is drawing attention in quality assurance of heterogeneous systems whose complexities are beyond most verification techniques' scalability. In this paper we introduce the idea of causality aid in falsification: by providing a falsification solver -- that relies on stochastic optimization of a certain cost function -- with suitable causal information expressed by a Bayesian network, search for a falsifying input value can be efficient. Our experiment results show the idea's viability.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{L. Bulwahn, M. Kamali, S. Linker (Eds.): First Workshop on\\ Formal Verification of Autonomous Vehicles (FVAV 2017).\\
EPTCS 257, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.257.2}{10.4204/EPTCS.257.2}}
\pdfoutput=1

